Privacy-Preserving Text Sanitization for Distributed Agents Collaboration via Disentangled Representations

When distributed agents exchange text across organizational boundaries, privacy leakage arises not only from explicit identifiers but also from distributional signatures such as formatting conventions, vocabulary choices, and syntactic patterns. We propose DiSan(Disentangled Sanitization), a privacy-preserving sanitization framework and a built-in component of Intern-Shannon for multi-agent collaboration. DiSan uses a two-stream encoder to factorize text into a source-invariant role subspace that preserves task semantics and a source-identifying style subspace that remains local. Federated proto-type alignment and adversarial regularization enable joint training without centralizing raw text. Experiments show that identifier-level masking is insufficient: masking 19.2% of tokens reduces TF-IDF stylometric attribution by only 18.6%. By contrast, DiSan reduces answer-level PII exposure by 20 times while maintaining 83% answer faithfulness on a distributed multi-agent RAG benchmark, and lowers Enron stylometric attribution by 73.2% under TF-IDF and 70.6% under a neural probe.

==> sections/impact_statement.tex <==
\section*{Impact Statement}
This paper presents work whose goal is to advance the field of Machine Learning, specifically in enabling privacy-preserving text sharing across distributed agent systems. There are potential positive societal consequences: our work could enable organizations to deploy collaborative agents more effectively while protecting sensitive data, which is particularly important in domains like healthcare and finance.

We also acknowledge potential risks. Privacy-preserving technologies could theoretically provide false assurance if deployed without proper threat modeling, or could be misused to obscure accountability. The honest-but-curious assumption may not hold in adversarial settings. We encourage practitioners to conduct domain-specific security audits before deployment.

Our main experiments use synthetic data with no real personal information. For external validation, we use the publicly available Enron email corpus, a standard benchmark for authorship attribution research that was released as part of the 2001 federal investigation and has been widely used in academic research for over two decades.


